A depolarisation census of ASKAP fast radio bursts

Fast radio bursts (FRBs) are luminous, dispersed pulses of extra-galactic origin. The physics of the emission mechanism, the progenitor environment, and their origin are unclear. Some repeating FRBs are observed to have frequency-dependent exponential suppression in linear polarisation fraction. This has been attributed to multipath propagation in a surrounding complex magneto-ionic environment. The magnitude of depolarisation can be quantified using the parameter $\rm \sigma^{\prime}_{RM}$, which can be used to model the magneto-ionic complexity of the medium. In addition to depolarisation, some repeating sources (in particular those with active magneto-ionic environments) have been identified to have co-located persistent radio sources (PRS). Searches for depolarisation of non-repeating sources are challenging due to the limited bandwidth of most FRB detection systems used to detect one-off bursts. However, even with a limited bandwidth, such depolarisation can be identified if it lies within the $\rm \sigma^{\prime}_{RM}$ sensitivity window of the telescope. In this paper, we present a search for depolarisation in $12$ one-off FRBs detected by the Australian SKA Pathfinder. We report on the first strongly depolarised FRB detected by ASKAP (FRB$~$20230526A) and a marginal detection of depolarisation in a second. We also report constraints on the presence of a PRS coincident with FRB$~$20230526A using observations obtained with the Australia Telescope Compact Array. We use this to study the relationship between $\rm \sigma^{\prime}_{RM}$ and PRS luminosity. Our investigation supports a scenario in which repeaters and non-repeaters share a common origin and where non-repeaters represent an older population relative to repeating FRBs.

==> FRB_properties.tex <==
\begin{table*}
	\begin{center}\renewcommand{\arraystretch}{1.5}%
		\begin{tabular}{ c c c c c c c c c c c c c}
			\hline
			\thead{FRB \\ (TNS)}  & \thead{DM$^\dag$ \\ (pc cm$^{-3}$)} & \thead{RM$^\ddag$ \\ (rad m$^{-2}$)} & z$^\dag$ & \thead{\sigmapRM$^{||}$ \\ (rad m$^{-2}$)} & P$_{\rm int}$$^{||}$ & \thead{\sigmaRM$^{||}$ \\ (rad m$^{-2}$)} & \thead{$\nu_{\rm centre}$$^{\dag}$ \\ (MHz)} & \thead{$\delta\nu$$^{||}$ \\ (MHz)} & \thead{$\tau$$^{||}$ \\ (ms)} & \thead{M1$^{||}$ \\ (log$_{10}$)} & \thead{M1.1$^{||}$ \\ (log$_{10}$)} & \thead{M2$^{||}$ \\ (log$_{10}$)}\\
			\hline

			20191228A & 380.1(2) & -13.9$\pm$0.8 & 0.243 & $<$5.22 & 0.93$^{+0.05}_{-0.05}$ & $<$4.0 & 1272 & 20.978 & 5.5$^{+0.2}_{-0.2}$ & 2.4 & 1.7 & 2.3 \\
 
			
			20200430A & 294(1) & 195.3$\pm$0.7 & 0.161 & $<$4.71 & 0.63$^{+0.22}_{-0.15}$ & $<$3.82 & 864 & 20.978 & 7.7$^{+0.5}_{-0.5}$ & 0.1 & 0.2 & 0.7\\
			
			20210117A & 398.3(7) & -43.7$\pm$0.8 & 0.214 & $<$2.48 & 0.97$^{+0.02}_{-0.02}$ & $<$1.74 & 1272 & 20.978 & 0.13$^{+0.1}_{-0.09}$ & 6.9 & 5.8 & 6.8\\
			
			20210320A & 384.8(3) & -289.3$\pm$0.1 & 0.2797  & 1.8$^{+0.08}_{-0.08}$ & 0.97$^{+0.02}_{-0.03}$ & 1.59$^{+0.17}_{-0.24}$ & 864 & 20.978 & 0.25$^{+0.0}_{-0.0}$  & 8 & 6.9 & 5.5\\
			
			20210407E & 251.9(2) & 10$\pm$1 & no host & $<$4.02 & 0.92$^{+0.05}_{-0.04}$ & $<$3.13 & 1272 & 20.978 & 0.09$^{+0.01}_{-0.01}$ & 3.7 & 3.1 & 3.9\\
			
			20210912A & 234.83(8) & 7.1$\pm$0.2 & no host & $<$3.88 & 0.57$^{+0.02}_{-0.01}$ & $<$2.99 & 1272 & 20.978 & 0.2$^{+0.2}_{-0.45}$ & -30.1 & 10.5 & 11.3 \\
			
			20220501C & 727(2) & -35.9$\pm$0.3 & 0.381 & $<$2.64 & 0.63$^{+0.06}_{-0.05}$ & $<$1.75 & 864 & 20.978 & 1.72$^{+0.71}_{-0.72}$ & 0.1 & 2.2 & 3.2 \\
			
			20220610A & 290.4(3) & 215.0$\pm$2 & 1.016 & $<$1.7 & 0.99$^{+0.01}_{-0.01}$ & $<$1.21 & 1272 & 20.978 & 0.46$^{+0.05}_{-0.07}$ & 1.5 & -0.1 & 0.9\\
			
			20220725A & 656.8(4) & 25.2$\pm$0.6 & 0.193 & $<$4.33 & 0.74$^{+0.13}_{-0.08}$ & $<$3.39 & 920 & 20.978 & 2.35$^{+0.11}_{-0.1}$ & 0.8 & 1 & 1.5\\
			
			20221106A & 640.2(5) & -447.0$\pm$1 & 0.204 & $<$10.18 & 0.93$^{+0.05}_{-0.07}$ & $<$9.42 & 1632 & 20.978 & - & 7.9 & 7 & 6.7\\

                20230526A & 361.4(2) & -613.0$\pm$2.0 & 0.157 & 12.61$^{+0.26}_{-0.24}$ & 0.8$^{+0.11}_{-0.12}$ & 11.25$^{+0.83}_{-1.1}$ & 1272 & 20.978 & 1.26$^{+0.04}_{-0.05}$ & 9.6 & 9.6 & 3.8\\

			20230718A & 477.0(5) & -243.1$\pm$0.9 & 0.0357 & $<$3.02 & 0.93$^{+0.03}_{-0.02}$ & $<$2.16 & 1272 & 20.978 & - & 6 & 6 & 7\\
			\hline
		\end{tabular}
	\end{center}
 	\caption{Depolarisation properties of the ICS FRB sample. The FRB TNS name, DM, RM, host redshift, \sigmapRM, \sigmaRM, P$_{\rm int}$, centre frequency $\nu$, the frequency resolution used for depolarisation model fit $\delta \nu$, and the scattering timescale $\tau$ for the ICS FRB sample are reported here. We report the log$_{10}$ Bayes evidence for Burn's law, the modified Burn's law, and the constant depolarisation models as M1, M1.1, and M2, respectively. The values for columns marked with $^\dag$ are parameters from \protect\cite{Shannon:2024}. The columns marked with $^{||}$ are the parameters derived in this work. $\ddag$RMs for the bursts are derived from Scott et al. 2024 (in prep). We use simple boxcar for FRBs where no scattering timescale are provided.}

    \label{tab:comparision_table}
\end{table*}



==> FRB_properties_update.tex <==
\begin{table*}
	\begin{center}\renewcommand{\arraystretch}{1.5}%
		\begin{tabular}{ c c c c c c c c c c c c c}
			\hline
			\thead{FRB \\ (TNS)}  & \thead{DM$^\dag$ \\ (pc cm$^{-3}$)} & \thead{RM$^\ddag$ \\ (rad m$^{-2}$)} & z$^\dag$ & \thead{\sigmapRM$^{||}$ \\ (rad m$^{-2}$)} & P$_{\rm int}$$^{||}$ & \thead{\sigmaRM$^{||}$ \\ (rad m$^{-2}$)} & \thead{$\nu_{\rm centre}$$^{\dag}$ \\ (MHz)} & \thead{$\delta\nu$$^{||}$ \\ (MHz)} & \thead{$\tau$$^{||}$ \\ (ms)} & \thead{Bayes Factor$^{||}$ \\ (log$_{10}$)} \\
            \hline
            20191228A &  380.1(2) & -13.9$\pm$0.8 & 0.243 & $<$5.22 & 0.93$^{+0.05}_{-0.05}$ & $<$4.0 & 1272 & 20.978 & 5.5$^{+0.2}_{-0.2}$ & -0.600 \\
            %\hline
            20200430A &  294(1) & 195.3$\pm$0.7 & 0.161 & $<$4.71 & 0.63$^{+0.22}_{-0.15}$ & $<$3.82 & 864 & 20.978 & 7.7$^{+0.5}_{-0.5}$ & -0.500 \\
            %\hline
            20210117A &  398.3(7)  & -43.7$\pm$0.8 & 0.214 & $<$2.48 & 0.97$^{+0.02}_{-0.02}$ & $<$1.74 & 1272 & 20.978 & 0.13$^{+0.1}_{-0.09}$ & -1 \\
            %\hline
            20210320A & 384.8(3) & -289.3$\pm$0.1 & 0.2797 & 1.8$^{+0.08}_{-0.08}$ & 0.97$^{+0.02}_{-0.03}$ & 1.59$^{+0.17}_{-0.24}$ & 864 & 20.978 & 0.25$^{+0.0}_{-0.0}$ & 1.400 \\
            %\hline
            20210407E &  251.9(2) & 10$\pm$1 & no host & $<$4.02 & 0.92$^{+0.05}_{-0.04}$ & $<$3.13 & 1272 & 20.978 & 0.09$^{+0.01}_{-0.01}$ & -0.800 \\
            %\hline
            20210912A &  234.83(8) & 7.1$\pm$0.2 & no host & $<$3.88 & 0.57$^{+0.02}_{-0.01}$ & $<$2.99 & 1272 & 20.978 & 0.2$^{+0.2}_{-0.45}$ & -0.800 \\
            %\hline
            20220501C &  727(2) & -35.9$\pm$0.3 & 0.381 & $<$2.64 & 0.63$^{+0.06}_{-0.05}$ & $<$1.75 & 864 & 20.978 & 1.72$^{+0.71}_{-0.72}$ & -1 \\
            %\hline
            20220610A &  290.4(3) & 215.0$\pm$2 & 1.016 & $<$1.7 & 0.99$^{+0.01}_{-0.01}$ & $<$1.21 & 1272 & 20.978 & 0.46$^{+0.05}_{-0.07}$ & -1 \\
            %\hline
            20220725A &  656.8(4) & 25.2$\pm$0.6 & 0.193 & $<$4.33 & 0.74$^{+0.13}_{-0.08}$ & $<$3.39 & 920 & 20.978 & 2.35$^{+0.11}_{-0.1}$ & -0.500 \\
            %\hline
            20221106A &  640.2(5) & -447.0$\pm$1 & 0.204 & $<$10.18 & 0.93$^{+0.05}_{-0.07}$ & $<$9.42 & 1632 & 20.978 & - & 0.300 \\
            %\hline
            20230526A &  361.4(2) & -613.0$\pm$2.0 & 0.157 & 12.61$^{+0.26}_{-0.24}$ & 0.8$^{+0.11}_{-0.12}$ & 11.25$^{+0.83}_{-1.1}$ & 1272 & 20.978 & 1.26$^{+0.04}_{-0.05}$ & 5.800 \\
            %\hline
            20230718A &  477.0(5) & -243.1$\pm$0.9 & 0.0357 & $<$3.02 & 0.93$^{+0.03}_{-0.02}$ & $<$2.16 & 1272 & 20.978 & - & -1 \\
            \hline

		\end{tabular}
	\end{center}
        \caption{Depolarisation properties of ICS FRB sample. The FRB TNS name, DM, RM, host redshift, \sigmapRM, \sigmaRM, P$_{\rm int}$, centre frequency $\nu$, the frequency resolution used for depolarisation model fit $\delta \nu$, and the scattering timescale $\tau$ for the ICS FRB sample are reported here. We report the log$_{10}$ Bayes Factor (BF) for the modified Burn's law and the constant depolarisation models. The higher positive value indicates higher preference to the modified Burn's law. The values for columns marked with $^\dag$ are parameters from \protect\cite{Shannon:2024}. The columns marked with $^{||}$ are the parameters derived in this work. $\ddag$RMs for the bursts are derived from Scott et al. 2025 (in prep). We use simple boxcar for FRBs where no scattering timescale are provided.}
 	%\caption{Depolarisation properties of ICS FRB sample. The FRB TNS name, DM of the FRB, RM of the FRB, redshift, \sigmapRM, \sigmaRM, P$_{\rm int}$, centre frequency $\nu$, thre frequency resolution used for depolarisation model fit $\delta \nu$, and the scattering timescale $\tau$ for the ICS FRB sample is reported here. We report the log$_{10}$ Bayes evidence for Burn's law, the modified Burn's law, and the constant depolarisation models as M1, M1.1, and M2, respectively. The values for columns marked with $^\dag$ are parameters from \protect\cite{Shannon:2024}. The columns marked with $^{||}$ are the parameters derived in this work. $\ddag$RMs for the bursts are derived from Scott et al. 2024 (in prep). We use simple boxcar for FRBs where no scattering timescale are provided.}

    \label{tab:comparision_table}
\end{table*}


